A Redundancy Reduction Approach for Controllable Sequential Recommendations

Sequential recommendation must operate under long-tailed item distributions and popularity-driven concentration, often forcing practitioners to trade short-list accuracy against long-tail exposure. In this work, we study feature decorrelation as a mechanism for shaping representation geometry in dot-product sequential recommenders, and analyze how this, in turn, affects popularity-driven concentration. We propose a decorrelation-regularized training framework that augments next-item prediction with an auxiliary redundancy-reduction term, and instantiate it with BT-SR, which uses the Barlow Twins objective. To form label-consistent positive pairs without synthetic corruptions, we pair user histories that share the same next-item target. Beyond accuracy, we provide a geometric analysis showing how decorrelation suppresses shared low-rank directions in the user representation space that can give popular items a global scoring advantage, and we introduce a bucket-based alignment concentration metric to quantify this effect. Experiments on five public benchmarks show that BT-SR consistently improves next-item ranking quality, while the decorrelation strength acts as a simple control knob that reallocates accuracy across head and tail items, enabling accuracy-exposure trade-offs. Our analysis also reveals that the impact on head-vs-tail exposure differs across datasets, reflecting interactions between decorrelation and data temporal structure.

==> recsys26-115/Source/tables/ablation_buckets_fig.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_1_buckets_hr.png}
    \caption{Sensitivity Analysis w.r.t. $ \alpha $ for recommendations over 3 item popularity buckets}
    \label{figure:ablation_alpha_buckets}
\end{figure*}

==> recsys26-115/Source/tables/ablation_lambda_buckets_fig.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_2_buckets_hr.png}
    \caption{Sensitivity Analysis w.r.t. $ \lambda $ for recommendations over 3 item popularity buckets}
    \label{figure:ablation_lambda_buckets}
\end{figure*}

==> recsys26-115/Source/tables/ablation_lambda_main_fig.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_2_HR.png}
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_2_cov.png}
    \caption{Sensitivity Analysis w.r.t. $ \lambda $ of hr@K and cov@K metrics }
    \label{figure:ablation_lambda_main}
\end{figure*}

==> recsys26-115/Source/tables/ablation_main_fig.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_1_HR.png}
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_1_cov.png}
    \caption{Sensitivity Analysis w.r.t. $ \alpha $ of hr@K and cov@K metrics }
    \label{figure:ablation_main}
\end{figure*}

==> recsys26-115/Source/tables/ablation_table.tex <==
\begin{table}[!t]
\caption{Ablation on item-wise sequence augmentations (as in CL4SRec) and replacing the SSL objective with SimSiam.}
{\footnotesize
\begin{tabular}{rlcccc}
\toprule
Dataset & Metric
& \begin{tabular}{@{}c@{}}SasRec \\ (CE baseline)\end{tabular}
& \begin{tabular}{@{}c@{}}SasRec \\ (CL4SRec aug.)\end{tabular}
& \begin{tabular}{@{}c@{}}SasRec \\ (SimSiam)\end{tabular}
& \begin{tabular}{@{}c@{}}BT-SR \\ {[}Ours{]}\end{tabular} \\
\midrule

\multirow{7}{*}{\rotatebox{90}{Yelp}}
 & hr@1    
 & 0.0043 
 & 0.0045
 & \underline{0.0047} 
 & \textbf{0.0049} \\

 & ndcg@5  
 & 0.0088 
 & 0.0102 
 & \underline{0.0108} 
 & \textbf{0.0117} \\

 & ndcg@10 
 & 0.0127 
 & 0.0137 
 & \underline{0.0143} 
 & \textbf{0.0150} \\

 & cov@1   
 & \textbf{0.0233} 
 & \textbf{0.0233} 
 & \underline{0.0225} 
 & 0.0218 \\

 & cov@5   
 & 0.0621 
 & \textbf{0.0658} 
 & \underline{0.0642} 
 & 0.0636 \\

 & cov@10  
 & 0.0911 
 & \textbf{0.1009} 
 & 0.0791 
 & \underline{0.0998} \\

\arrayrulecolor{gray!30}\cmidrule(lr){2-6}\arrayrulecolor{black}

\multirow{7}{*}{\rotatebox{90}{Kindle}}
 & hr@1    
 & 0.0533 
 & 0.0539 
 & \underline{0.0546} 
 & \textbf{0.0565} \\

 & ndcg@5  
 & 0.0726 
 & 0.0731 
 & \underline{0.0740} 
 & \textbf{0.0755} \\

 & ndcg@10 
 & 0.0765 
 & 0.0786 
 & \underline{0.0789} 
 & \textbf{0.0796} \\

 & cov@1   
 & 0.0409 
 & \textbf{0.0439} 
 & 0.0425 
 & \underline{0.0433} \\

 & cov@5   
 & 0.1492 
 & \underline{0.1602} 
 & 0.1560 
 & \textbf{0.1656} \\

 & cov@10  
 & 0.2346 
 & \underline{0.2565} 
 & 0.0785 
 & \textbf{0.2665} \\

\bottomrule
\end{tabular}
}
\label{tab:abl}
\end{table}


==> recsys26-115/Source/tables/buckets_fig.tex <==
\begin{figure}[!t]
    \centering

    % ─── first row ─────────────────────────────────────────────
    \includegraphics[width=0.5\linewidth]{pictures/bucket_metrics/ml.png}
    \includegraphics[width=0.49\linewidth]{pictures/bucket_metrics/ml_hr10.png}
    \\[-30pt]
    
    \includegraphics[width=0.5\linewidth]{pictures/bucket_metrics/yelp_hr1_alt.png}
    \includegraphics[width=0.49\linewidth]{pictures/bucket_metrics/yelp_hr10.png}
    \\[-30pt]
    
    \includegraphics[width=0.5\linewidth]{pictures/bucket_metrics/gowalla.png}
    \includegraphics[width=0.49\linewidth]{pictures/bucket_metrics/gowalla_hr10.png}
    \\[-32pt]
    
    \caption{HR@1 (left) and HR@10 (right) metrics for the three item-popularity buckets across three datasets.}
    \label{figure:pop_buckets}
    %\\[-20pt]
    \Description[Grouped bar charts comparing HR@1 (left) and HR@10 (right) for baseline models: SASRec(CE), SASRec(SCE), DuoRec, and our BT-SR across head, mid, and tail item-popularity buckets on three datasets.]{Figure 1 contains two grouped bar-chart panels. The left panel shows HR@1 and the right panel shows HR@10, each broken down by three item-popularity buckets (head/most popular, mid, and tail/least popular) for three datasets. Bars compare the baseline models: SASRec(CE), SASRec(SCE) and DuoRec, against the proposed BT-SR model. Across datasets, BT-SR is slightly below the baseline in the head bucket for HR@1 but clearly higher for the mid and tail buckets, indicating improved personalization on less popular items. For HR@10, BT-SR matches or exceeds the baseline even in the head bucket, showing that its overall ranking accuracy is not sacrificed while long-tail items are surfaced more often.}
\end{figure}

==> recsys26-115/Source/tables/compare_buckets.tex <==
\begin{figure}[!t]
    \centering

    % ─── first row ─────────────────────────────────────────────
    % \vspace{-1em}
    \includegraphics[width=0.5\linewidth]{pictures/bucket_metrics/modes_yelp_hr_1.png}
    \includegraphics[width=0.49\linewidth]{pictures/bucket_metrics/modes_yelp_hr_10.png}
    \vspace{-4em}
    \caption{Performance comparison on the Yelp dataset under two regimes: BT-SR with $\alpha=0.1$ favors popular items (high HR@1), while BT-SR(*) with $\alpha=0.4$ promotes diverse, less popular items early in the list, boosting personalization and maintaining high overall accuracy (HR@10).}
    \label{figure:pop_buckets_modes}
    %\\[-20pt]
    \Description[Bar chart compares recommendation metrics on Yelp for BT-SR at $\alpha=0.1$ (head-favoring), BT-SR(*) at $\alpha=0.4$ (tail-favoring) and SASRecc(SCE), across HR@1, and HR@10.]{Figure 4 shows a bar chart for the Yelp dataset comparing two configurations of BT-SR: one with $\alpha=0.1$, which favors popular items and achieves the highest HR@1, and another labeled BT-SR(*) with $\alpha=0.4$, which promotes less popular items earlier in the ranked list, and SASRec(SCE). The chart displays HR@1 and HR@10 side by side for both configurations, showing that the $\alpha=0.4$ setting sacrifices some head-item precision (lower HR@1) but improves personalization and diversity while keeping HR@10 comparably high, demonstrating the practical trade-off enabled by tuning $\alpha$.}

\end{figure}


==> recsys26-115/Source/tables/compare_buckets_table.tex <==
\begin{table}[!t]
    \centering
    \caption{Integral metric for Figure 4}
    \begin{tabular}{c|c c c}
        \toprule
          & SASRec(BCE) & BT-SR( $ \alpha = 0.1 $ ) & BT-SR( $ \alpha = 0.4 $ ) \\ 
         \toprule
         \textbf{ndcg@20} & 0.0176 & 0.0180 & 0.0182 \\
         \toprule
    \end{tabular}
    \label{tab:pop_buckets_ndcg}
\end{table}

==> recsys26-115/Source/tables/mixed_fig.tex <==
\begin{figure}[!t]
    \centering

    \includegraphics[width=0.5\linewidth]{pictures/scores_density/MovieLens_1M.png}
    \includegraphics[width=0.49\linewidth]{pictures/spectrum/MovieLens_1M.png}
    
    \includegraphics[width=0.49\linewidth]{pictures/scores_density/YELP.png}
    \includegraphics[width=0.49\linewidth]{pictures/spectrum/YELP.png}
    
    \includegraphics[width=0.5\linewidth]{pictures/scores_density/Gowalla.png}
    \includegraphics[width=0.49\linewidth]{pictures/spectrum/Gowalla.png}
    
    \caption{(left) Comparison of score density distributions for positive and negative candidate pairs across three datasets. We quantify model’s confidence in distinguishing relevant candidates by the histogram overlap factor (\emph{Overlap})—lower values indicate better separation. (right) Singular value spectra of the sequence embeddings for each dataset, annotated with their computed effective ranks (in legend), illustrate the effective dimensionality of the learned representations. }
    \label{figure:scores_dens_fig}
    %\\[-10pt]
\end{figure}

==> recsys26-115/Source/tables/ml_abla.tex <==
\begin{figure}[!t]
    \centering

    % ─── first row ─────────────────────────────────────────────
    % \begin{minipage}[t]{0.49\linewidth}
    %   \includegraphics[width=\linewidth]{pictures/ablation/ML1M_lambda_1_cov.png}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.49\linewidth}
    %   \includegraphics[width=\linewidth]{pictures/ablation/ML1M_lambda_1_buckets_hr.png}
    % \end{minipage}
    \includegraphics[width=1\linewidth]{pictures/ablation/alpha_diversity_tradeoff.png}
    %\includegraphics[width=0.49\linewidth]{pictures/ablation/ML1M_lambda_1_buckets_hr.png}
    
    \caption{Effect of the trade-off parameter $\alpha$ on accuracy (HR@10) and coverage (COV@10) for YELP and MovieLens-1M.
Results are reported over the full catalog, along with relative changes of HR@10 across three popularity buckets (w.r.t. balance point).
Varying $\alpha$ induce head-oriented, balanced, and tail-oriented recommendation regimes. }
    \label{figure:ml_abol}
    \Description[Line plots showing HR@10 and COV@10 as functions of the decorrelation weight $\alpha$ for Yelp and MovieLens-1M, plus relative HR@10 change across three popularity buckets.]{Figure 3 presents line charts with the decorrelation strength $\alpha$ (ranging from 0 to 0.5) on the x-axis, shown separately for Yelp and MovieLens-1M. For each dataset, one curve shows HR@10 and another shows COV@10 (item coverage), both computed over the full catalog as $\alpha$ increases. An additional set of curves shows the relative change in HR@10 for the head, mid, and tail popularity buckets relative to a chosen 'balance point' value of $\alpha$.

For Yelp, increasing $\alpha$ beyond the balance point produces a steady rise in COV@10, while HR@10 declines only moderately. The bucket-wise curves for Yelp show substantial HR@10 gains for the least-frequent (tail) items and only mild losses for the most-frequent (head) items, indicating that stronger decorrelation shifts recommendation mass toward long-tail items while preserving competitive overall accuracy.

For MovieLens-1M, the pattern differs: the best COV@10 is achieved at small $\alpha$ values, while larger $\alpha$ reduces both HR@10 and COV@10. The bucket-wise breakdown for MovieLens-1M shows that this degradation is concentrated in the medium- and low-frequency groups, whereas HR@10 for the most frequent items actually improves as $\alpha$ grows — the opposite direction from Yelp's trend.

Together, the two datasets illustrate that $\alpha$ acts as a tunable knob that reshapes the head-tail allocation of recommendation accuracy, but the direction and magnitude of this trade-off is dataset-dependent, likely reflecting differences in interaction sparsity and timestamp/popularity structure between Yelp and MovieLens-1M.}
\end{figure}

==> recsys26-115/Source/tables/ml_alignment.tex <==
\begin{figure}[!t]
    \centering

    % ─── first row ─────────────────────────────────────────────
    \includegraphics[width=1\linewidth]{pictures/alignment/rel_align_3.png}
    %\includegraphics[width=0.49\linewidth]{pictures/ablation/yelp_lambda_1_buckets_hr.png}
    
    \caption{
    Alignment Concentration on Movielens-1M, Yelp and Gowalla datasets. (left) We plot each model in relative alignment, $\tilde g_b$, coordinates. (right) The AC score quantifies, across all tail buckets, how much the alignment of less popular items falls short of the alignment of head-bucket items.}
    \label{figure:ml_alignment}
    \Description[Left: radar plots of relative head-normalized alignment across three popularity buckets for BT-SR, SASRec(CE), SASRec(SCE) and DuoRec models on MovieLens-1M, Yelp, and Gowalla. Right: bar chart of the Alignment Concentration (AC) score per model per dataset, with BT-SR showing the lowest values.]{Figure 2 has two parts. The left part shows three radar (spider) plots, one per dataset (MovieLens-1M, Yelp, Gowalla), where each axis corresponds to one of three item-popularity buckets and each colored line represents a different model (SASRec-CE, SASRec-SCE, DuoRec, BT-SR, etc.). The head bucket is normalized to 1, and the plotted values ($g_b$) show how strongly items in the mid and tail buckets align with the shared low-rank user-representation subspace relative to the head. BT-SR's line is visibly flatter or extends beyond 1 in the outer buckets compared to competing models, meaning it is less head-concentrated. The right part is a grouped bar chart showing the scalar Alignment Concentration (AC) score for each model on each dataset; lower values indicate weaker head-item dominance. BT-SR consistently has the lowest (or most negative) AC score across all three datasets, confirming it reduces reliance on shared low-rank directions that favor popular items.}
\end{figure}



==> recsys26-115/Source/tables/old_met.tex <==
\begin{table*}[!ht]
    \caption{Performance comparison across all datasets.Bold scores are the best on the dataset for the given metric,underlined scores are the second best.}
    {\tiny
    \begin{tabular}{rlcccccccl}
    \toprule
    Dataset & Metric & SasRec(BCE) & SasRec(CE) & SasRec(SCE) & CL4SRec & DuoRec & EC4SRec & BT-SR & Improve \\
    \midrule
    \multirow{9}{*}{ML 1M}
     & hr@1 & 0.0160 & \underline{0.0213} & 0.0200 & 0.0182 & 0.0200 & 0.0213 & \textbf{0.0293} & +37.6\% \\
     & hr@5   & 0.0493 & 0.0600 & \underline{0.0587} & 0.0476 & 0.0480 & 0.0534 & \textbf{0.0600} & +0.0\%  \\
     & hr@10  & 0.0893 & 0.0880 & \underline{0.0933} & 0.0834 & 0.0800 & 0.0880 & \textbf{0.0987} & +5.8\%  \\
     & ndcg@5 & 0.0319 & \underline{0.0404} & 0.0393 & 0.0342 & 0.0353 & 0.0364 & \textbf{0.0461} & +14.1\% \\
     & ndcg@10& 0.0443 & 0.0494 & \underline{0.0503} & 0.0464 & 0.0456 & 0.0492 & \textbf{0.0583} & +15.9\% \\
     & ndcg@50& 0.0799 & \underline{0.0818} & 0.0800 & 0.0712 & 0.0723 & 0.0748 & \textbf{0.0871} & +6.5\%  \\
     & cov@1  & 0.0320 & \underline{0.0887} & \textbf{0.0961} & 0.0335 & 0.0361 & 0.0387 & 0.0849 & -11.7\% \\
     & cov@5  & 0.1473 & 0.2265 & \textbf{0.2568} & 0.0969 & 0.0936 & 0.1002 & \underline{0.2327} & -9.4\% \\
     & cov@10 & 0.2434 & 0.3185 & \textbf{0.3645} & 0.1329 & 0.1459 & 0.1591 & \underline{0.3242} & -11.1\% \\
    \midrule
    \multirow{9}{*}{YELP}
     & hr@1   & \underline{0.0045} & 0.0043 & 0.0040 & 0.0028 & 0.0027 & 0.0028 & \textbf{0.0049} & +8.9\% \\
     & hr@5   & \underline{0.0162} & 0.0137 & 0.0152 & 0.0087 & 0.0094 & 0.0090 & \textbf{0.0183} & +13.0\% \\
     & hr@10  & 0.0292 & 0.0257 & 0.0277 & 0.0192 & 0.0188 & \underline{0.0199} & \textbf{0.0288} & -1.4\% \\
     & ndcg@5 & \underline{0.0104} & 0.0088 & 0.0097 & 0.0060 & 0.0061 & 0.0062 & \textbf{0.0117} & +12.5\% \\
     & ndcg@10& \underline{0.0146} & 0.0127 & 0.0137 & 0.0085 & 0.0091 & 0.0092 & \textbf{0.0150} & +2.7\%  \\
     & ndcg@50& \textbf{0.0280} & 0.0263 & 0.0258 & 0.0178 & 0.0172 & \underline{0.0184} & 0.0267 & -4.6\%  \\
     & cov@1  & 0.0103 & \textbf{0.0233} & 0.0135 & 0.0057 & 0.0059 & 0.0059 & \underline{0.0218} & -6.4\%  \\
     & cov@5  & 0.0333 & \underline{0.0621} & 0.0413 & 0.0170 & 0.0161 & 0.0171 & \textbf{0.0636} & +2.4\%  \\
     & cov@10 & 0.0541 & \underline{0.0911} & 0.0661 & 0.0276 & 0.0255 & 0.0275 & \textbf{0.0998} & +9.5\% \\
    \midrule
    \multirow{9}{*}{Gowalla}
     & hr@1   & 0.0173 & 0.0143 & \underline{0.0196} & 0.0157 & 0.0144 & 0.0142 & \textbf{0.0205} & +4.6\%  \\
     & hr@5   & 0.0506 & 0.0431 & \underline{0.0548} & 0.0433 & 0.0473 & 0.0440 & \textbf{0.0592} & +8.0\%  \\
     & hr@10  & 0.0756 & 0.0660 & \underline{0.0811} & 0.0694 & 0.0712 & 0.0757 & \textbf{0.0851} & +4.9\%  \\
     & ndcg@5 & 0.0339 & 0.0289 & \underline{0.0372} & 0.0318 & 0.0310 & 0.0331 & \textbf{0.0400} & +7.5\%  \\
     & ndcg@10& 0.0419 & 0.0364 & \underline{0.0457} & 0.0411 & 0.0387 & 0.0397 & \textbf{0.0483} & +5.7\%  \\
     & ndcg@50& 0.0613 & 0.0528 & \underline{0.0640} & 0.0535 & 0.0587 & 0.0549 & \textbf{0.0667} & +4.2\%  \\
     & cov@1  & 0.0230 & 0.0228 & 0.0214 & 0.0252 & \underline{0.0255} & 0.0270 & \textbf{0.0321} & +25.9\% \\
     & cov@5  & 0.0892 & 0.0725 & 0.0921 & \underline{0.0950} & 0.0939 & 0.0998 & \textbf{0.1280} & +36.3\% \\
     & cov@10 & 0.1557 & 0.1153 & \underline{0.1625} & 0.1538 & 0.1595 & 0.1650 & \textbf{0.2187} & +34.6\% \\
    \midrule
    \multirow{9}{*}{Beauty}
     & hr@1   & 0.0179 & 0.0269 & \underline{0.0305} & 0.0292 & 0.0305 & 0.0312 & \textbf{0.0314} & +3.0\%  \\
     & hr@5   & 0.0538 & \underline{0.0591} & 0.0582 & 0.0555 & 0.0573 & 0.0574 & \textbf{0.0618} & +4.6\%  \\
     & hr@10  & 0.0789 & 0.0896 & \underline{0.0905} & 0.0830 & 0.0860 & 0.0815 & \textbf{0.0941} & +4.0\%  \\
     & ndcg@5 & 0.0355 & 0.0425 & \underline{0.0442} & 0.0412 & 0.0436 & 0.0455 & \textbf{0.0460} & +4.1\%  \\
     & ndcg@10& 0.0434 & 0.0524 & \underline{0.0543} & 0.0530 & 0.0527 & 0.0557 & \textbf{0.0563} & +3.7\%  \\
     & ndcg@50& 0.0659 & 0.0777 & \underline{0.0794} & 0.0833 & 0.0789 & 0.0794 & \textbf{0.0829} & +4.4\%  \\
     & cov@1  & 0.0620 & 0.0546 & 0.0499 & 0.0603 & \underline{0.0607} & \textbf{0.0679} & 0.0492 & -20.6\% \\
     & cov@5  & 0.2200 & 0.1782 & 0.1760 & \underline{0.2212} & 0.2100 & 0.2103 & \textbf{0.1562} & -29.0\% \\
     & cov@10 & 0.3448 & 0.2752 & 0.2766 & \underline{0.3362} & 0.3234 & 0.3236 & \textbf{0.2397} & -30.5\% \\
    \midrule
    \multirow{9}{*}{Kindle Store}
     & hr@1   & 0.0451 & 0.0471 & \underline{0.0533} & 0.0469 & 0.0471 & 0.0505 & \textbf{0.0565} & +6.0\%  \\
     & hr@5   & 0.0832 & 0.0813 & \underline{0.0899} & 0.0813 & 0.0762 & 0.0785 & \textbf{0.0916} & +1.9\%  \\
     & hr@10  & 0.0990 & 0.0965 & \underline{0.1022} & 0.0910 & 0.0897 & 0.0955 & \textbf{0.1043} & +2.1\%  \\
     & ndcg@5 & 0.0655 & 0.0652 & \underline{0.0726} & 0.0635 & 0.0625 & 0.0652 & \textbf{0.0755} & +4.0\%  \\
     & ndcg@10& 0.0705 & 0.0700 & \underline{0.0765} & 0.0662 & 0.0668 & 0.0672 & \textbf{0.0796} & +4.1\%  \\
     & ndcg@50& 0.0786 & 0.0803 & \underline{0.0852} & 0.0731 & 0.0771 & 0.0736 & \textbf{0.0886} & +4.0\%  \\
     & cov@1  & 0.0396 & 0.0337 & \underline{0.0409} & 0.0363 & 0.0356 & 0.0369 & \textbf{0.0433} & +5.9\%  \\
     & cov@5  & 0.1278 & 0.1076 & \underline{0.1492} & 0.1077 & 0.1123 & 0.1082 & \textbf{0.1656} & +11.0\% \\
     & cov@10 & 0.1920 & 0.1665 & \underline{0.2346} & 0.1598 & 0.1719 & 0.1703 & \textbf{0.2665} & +13.6\% \\
    \bottomrule
    \end{tabular}
    }
    \label{table:utility_metrics}
\end{table*}










\begin{figure*}[!t]
    \centering

    % ─── first row ─────────────────────────────────────────────
    \includegraphics[width=0.33\linewidth]{pictures/bucket_metrics/ml.png}
    \includegraphics[width=0.33\linewidth]{pictures/bucket_metrics/yelp.png}
    \includegraphics[width=0.32\linewidth]{pictures/bucket_metrics/gowalla.png}%
    \\[-40pt] % ← tighten vertical space (adjust value to taste)

    % ─── second row ────────────────────────────────────────────
    \includegraphics[width=0.33\linewidth]{pictures/bucket_metrics/ml_hr10.png}
    \includegraphics[width=0.33\linewidth]{pictures/bucket_metrics/yelp_hr10.png}
    \includegraphics[width=0.32\linewidth]{pictures/bucket_metrics/gowalla_hr10.png}
    \\[-40pt]
    
    \caption{Item-popularity-bucket HR@1 and HR@10 metrics across three datasets}
    \label{figure:pop_buckets}
\end{figure*}

==> recsys26-115/Source/tables/projections.tex <==
\begin{figure}[!t]
    %\\[-5pt]
    \centering
    \includegraphics[width=0.99\linewidth]{pictures/projections/seq_yelp.png}
    \includegraphics[width=0.99\linewidth]{pictures/projections/seq_ml1m.png}
    \caption{UMAP of sequence embeddings from BT-ST (ours), SasRec (CE; base model), and DuoRec (contrastive SR) on Yelp (top row) and MovieLens 1M (bottom row). On Yelp, BT-ST produces more dispersed, sparser clusters. On MovieLens 1M, it yields fewer, tighter clusters with higher density.}
    \label{figure:seq_2d_yelp}
    %\\[-15pt]
\end{figure}

==> recsys26-115/Source/tables/scores_dens_fig.tex <==
\begin{figure}[!ht]
    \centering

    \includegraphics[width=0.5\linewidth]{pictures/scores_density/MovieLens 1M.png}
    \includegraphics[width=0.5\linewidth]{pictures/spectrum/MovieLens 1M.png}
    
    \includegraphics[width=0.49\linewidth]{pictures/scores_density/YELP.png}
    \includegraphics[width=0.49\linewidth]{pictures/spectrum/YELP.png}
    
    \includegraphics[width=0.5\linewidth]{pictures/scores_density/Gowalla.png}
    \includegraphics[width=0.5\linewidth]{pictures/spectrum/Gowalla.png}
    
    \caption{Scores densities comparison for positives and negatives candidates on 3 datasets. To estimate confidence of relevant candidates we computed histograms overlap factor between positives and negatives(Overlap). Lower overlap is better }
    \label{figure:scores_dens_fig}
\end{figure}

==> recsys26-115/Source/tables/spectrum_fig.tex <==
\begin{figure}[!ht]
    \\[-10pt]
    \centering
    \includegraphics[width=0.5\linewidth]{pictures/spectrum/MovieLens 1M.png}
    \includegraphics[width=0.49\linewidth]{pictures/spectrum/YELP.png}
    \includegraphics[width=0.5\linewidth]{pictures/spectrum/Gowalla.png}
    
    \caption{Sequence embeddings singular values across multiple datasets with stable rank}
    \label{figure:spectrums}
\end{figure}

==> recsys26-115/Source/tables/utility_backbones.tex <==

\begin{table}[b]
\caption{NDCG@10 performance comparison of three SASRec variants (BCE loss, CE loss, SCE loss) with and without the Barlow Twins regularization term. Results highlight consistent improvements from Barlow Twins across all scenarios.}
\label{table:utility_backbones}
    {\footnotesize
        \begin{tabular}{rcc|cc|cc}
        \toprule
         & BCE & BCE + BT & CE & CE + BT & SCE & SCE + BT \\
        \midrule
        ML-1M & 0.0443 & \textbf{0.0490} & 0.0494 & \textbf{0.0583} & 0.0503 & \textbf{0.0562} \\
        YELP & 0.0146 & \textbf{0.0149} & 0.0127 & \textbf{0.0150} & 0.0137 & \textbf{0.0141} \\
        Gowalla & 0.0419 & \textbf{0.0434} & 0.0364 & \textbf{0.0481} & 0.0457 & \textbf{0.0483} \\
        Beauty & 0.0434 & \textbf{0.0440} & 0.0524 & \textbf{0.0563} & 0.0543 & \textbf{0.0549} \\
        Kindle Store & 0.0705 & \textbf{0.0733} & 0.0700 & \textbf{0.0746} & 0.0765 & \textbf{0.0796} \\
        \bottomrule
        \end{tabular}
    }
\end{table}

==> recsys26-115/Source/tables/utility_metrics.tex <==
\begin{table*}[!t]
    \caption{Performance comparison across all datasets. The best result in each row is highlighted in bold, the second-best result is underlined. All metrics are averaged over 5 independent runs,  statistically significant improvements are marked by (*).}
    {\footnotesize
    \begin{tabular}{rlcccccccccl}
    \toprule
    Dataset & Metric & SasRec(BCE) & SasRec(CE) & SasRec(SCE) & CL4SRec & DuoRec & EC4SRec & BT-PT & \textbf{BT-SR}(Ours) & Improve \\
    \midrule
    \multirow{9}{*}{ML-1M}
 & hr@1    & 0.0160                   & \underline{0.0213}       & 0.0200                   & 0.0182                   & 0.0200                   & \underline{0.0213}                   & 0.0200                   & \textbf{0.0240* $ \pm $ 0.0048} & +12.7\% \\
 & hr@5    & 0.0493                   & \underline{0.0600}       & 0.0587                   & 0.0476                   & 0.0480                   & 0.0534                   & 0.0573                   & \textbf{0.0639* $ \pm $ 0.0024} & +6.5\% \\
 & hr@10   & 0.0893                   & 0.0847                   & \underline{0.0933}       & 0.0834                   & 0.0800                   & 0.0880                   & 0.0893                   & \textbf{0.0945* $ \pm $ 0.0080} & +1.3\% \\
  \arrayrulecolor{gray!30}\cmidrule(lr){2-11}\arrayrulecolor{black}
 & ndcg@5  & 0.0319                   & \underline{0.0404}       & 0.0393                   & 0.0342                   & 0.0353                   & 0.0364                   & 0.0383                   & \textbf{0.0436* $ \pm $ 0.0020} & +7.9\% \\ 
 & ndcg@10 & 0.0443                   & 0.0494                   & \underline{0.0503}       & 0.0464                   & 0.0456                   & 0.0487                   & 0.0486                   & \textbf{0.0534* $ \pm $ 0.0037} & +6.2\% \\
\arrayrulecolor{gray!30}\cmidrule(lr){2-11}\arrayrulecolor{black}
 & cov@1   & 0.0320                   & \underline{0.0887}       & \textbf{0.0961}          & 0.0335                   & 0.0361                   & 0.0387                   & 0.0846                   & 0.0816* $ \pm $ 0.0035          & -15.1\% \\
 & cov@5   & 0.1473                   & 0.2265       & \textbf{0.2568}          & 0.0969                   & 0.0936                   & 0.1002                   & \underline{0.2267}        & 0.2223* $ \pm $ 0.0083          & -13.4\% \\
 & cov@10  & 0.2434                   & 0.3185                   & \textbf{0.3645}          & 0.1329                   & 0.1459                   & 0.1591                   & \underline{0.3193}        & 0.3189* $ \pm $ 0.0123          & -12.5\% \\

    \midrule
    \multirow{9}{*}{YELP}
 & hr@1   & \underline{0.0045} & 0.0043 & 0.0040 & 0.0028 & 0.0027 & 0.0028 & 0.0030 & \textbf{0.0049* $\pm$ 0.0005}  & +8.9\% \\
 & hr@5   & \underline{0.0162} & 0.0137 & 0.0152 & 0.0087 & 0.0094 & 0.0090 & 0.0121 & \textbf{0.0183* $\pm$ 0.0008}  & +13.0\% \\
 & hr@10  & \textbf{0.0292} & 0.0257 & 0.0277 & 0.0192 & 0.0188 & 0.0199 & 0.0244 & \underline{0.0288 $\pm$ 0.0010}  & –1.4\% \\
\arrayrulecolor{gray!30}\cmidrule(lr){2-11}\arrayrulecolor{black}
 & ndcg@5 & \underline{0.0104} & 0.0088 & 0.0097 & 0.0060 & 0.0061 & 0.0062 & 0.0074 & \textbf{0.0117* $\pm$ 0.0006}  & +12.5\% \\
 & ndcg@10& \underline{0.0146} & 0.0127 & 0.0137 & 0.0085 & 0.0091 & 0.0092 & 0.0114 & \textbf{0.0150* $\pm$ 0.0006}  & +2.7\%  \\
\arrayrulecolor{gray!30}\cmidrule(lr){2-11}\arrayrulecolor{black}
 & cov@1  & 0.0103 & \textbf{0.0233} & 0.0135 & 0.0057 & 0.0059 & 0.0059 & 0.0159 & \underline{0.0218 $\pm$ 0.0034}  & –6.4\%  \\
 & cov@5  & 0.0333 & \underline{0.0621} & 0.0413 & 0.0170 & 0.0161 & 0.0171 & 0.0444 & \textbf{0.0636* $\pm$ 0.0089}  & +2.4\%  \\
 & cov@10 & 0.0541 & \underline{0.0911} & 0.0661 & 0.0276 & 0.0255 & 0.0275 & 0.0678 & \textbf{0.0998* $\pm$ 0.0128}  & +9.5\% \\

    \midrule
    \multirow{9}{*}{Gowalla}
 & hr@1   & 0.0173 & 0.0143 & \underline{0.0196} & 0.0157 & 0.0144 & 0.0142 & 0.0184 & \textbf{0.0205* $\pm$ 0.0010} & +4.6\%  \\
 & hr@5   & 0.0506 & 0.0431 & \underline{0.0548} & 0.0433 & 0.0473 & 0.0440 & 0.0502 & \textbf{0.0592* $\pm$ 0.0010}  & +8.0\%  \\
 & hr@10  & 0.0756 & 0.0660 & \underline{0.0811} & 0.0694 & 0.0712 & 0.0757 & 0.0728 & \textbf{0.0851* $\pm$ 0.0020}  & +4.9\%  \\
\arrayrulecolor{gray!30}\cmidrule(lr){2-11}\arrayrulecolor{black}
 & ndcg@5 & 0.0339 & 0.0289 & \underline{0.0372} & 0.0318 & 0.0310 & 0.0331 & 0.0344 & \textbf{0.0400* $\pm$ 0.0009}  & +7.5\%  \\
 & ndcg@10& 0.0419 & 0.0364 & \underline{0.0457} & 0.0411 & 0.0387 & 0.0397 & 0.0417 & \textbf{0.0483* $\pm$ 0.0013}  & +5.7\%  \\
\arrayrulecolor{gray!30}\cmidrule(lr){2-11}\arrayrulecolor{black}
 & cov@1  & 0.0230 & 0.0228 & 0.0214 & 0.0252 & 0.0255 & 0.0270 & \textbf{0.0368} & \underline{0.0321* $\pm$ 0.0039}  & -12.8\% \\
 & cov@5  & 0.0892 & 0.0725 & 0.0921 & 0.0950 & 0.0939 & 0.0998 & \underline{0.1269} & \textbf{0.1280* $\pm$ 0.0140}  & +7.3\% \\
 & cov@10 & 0.1557 & 0.1153 & 0.1625 & 0.1538 & 0.1595 & 0.1650 & \underline{0.2037} & \textbf{0.2187* $\pm$ 0.0237}  & +7.6\% \\

    \midrule
    \multirow{9}{*}{Beauty}
 & hr@1    & 0.0179                   & 0.0269                   & \underline{0.0305}       & 0.0292                   & \underline{0.0305}       & 0.0303                   & 0.0278                   & \textbf{0.0326* $ \pm $ 0.0013} & +6.9\% \\
 & hr@5    & 0.0538                   & 0.0591       & 0.0582                   & 0.0555                   & 0.0573                   & 0.0574                   & \underline{0.0601}           & \textbf{0.0606* $ \pm $ 0.0025} & +2.5\% \\
 & hr@10   & 0.0789                   & 0.0896                   & 0.0905       & 0.0830                   & 0.0860                   & 0.0815                   & \underline{0.0928}           & \textbf{0.0937* $ \pm $ 0.0019} & +3.5\% \\
\arrayrulecolor{gray!30}\cmidrule(lr){2-11}\arrayrulecolor{black}
 & ndcg@5  & 0.0355                   & 0.0425                   & 0.0442                   & 0.0412                   & 0.0436                   & \underline{0.0455}       & 0.0441                   & \textbf{0.0463* $ \pm $ 0.0002} & +1.8\% \\
 & ndcg@10 & 0.0434                   & 0.0524                   & 0.0543                   & 0.0530                   & 0.0527                   & 0.0537                   & \underline{0.0551}        & \textbf{0.0569* $ \pm $ 0.0001} & +4.8\% \\
\arrayrulecolor{gray!30}\cmidrule(lr){2-11}\arrayrulecolor{black}
 & cov@1   & 0.0620                   & 0.0546                   & 0.0499                   & 0.0603                   & 0.0607                   & \textbf{0.0679}          & \underline{0.0634}        & 0.0491* $ \pm $ 0.0078          & -27.7\% \\
 & cov@5   & \underline{0.2200}       & 0.1782                   & 0.1760                   & \textbf{0.2212}          & 0.2100                   & 0.2103                   & 0.2130                   & 0.1532* $ \pm $ 0.0357          & -29.2\% \\
 & cov@10  & \textbf{0.3448}          & 0.2752                   & 0.2766                   & \underline{0.3362}       & 0.3234                   & 0.3236                   & 0.3272                   & 0.3234 $ \pm $ 0.0612          & -6.2\% \\

    \midrule
    \multirow{9}{*}{Kindle Store}
 & hr@1    & 0.0451                   & 0.0471                   & \underline{0.0533}       & 0.0469                   & 0.0471                   & 0.0505                   & 0.0502                   & \textbf{0.0564* $ \pm $ 0.0007} & +5.8\% \\
 & hr@5    & 0.0832                   & 0.0813                   & \underline{0.0899}       & 0.0813                   & 0.0762                   & 0.0785                   & 0.0820                   & \textbf{0.0903* $ \pm $ 0.0018} & +0.4\% \\
 & hr@10   & 0.0990                   & 0.0965                   & \underline{0.1022}       & 0.0910                   & 0.0897                   & 0.0955                   & 0.0953                   & \textbf{0.1058* $ \pm $ 0.0012} & +3.5\% \\
\arrayrulecolor{gray!30}\cmidrule(lr){2-11}\arrayrulecolor{black}
 & ndcg@5  & 0.0655                   & 0.0652                   & \underline{0.0726}       & 0.0635                   & 0.0625                   & 0.0652                   & 0.0678                   & \textbf{0.0747* $ \pm $ 0.0009} & +2.9\% \\
 & ndcg@10 & 0.0705                   & 0.0700                   & \underline{0.0765}       & 0.0662                   & 0.0668                   & 0.0672                   & 0.0721                   & \textbf{0.0796* $ \pm $ 0.0005} & +4.1\% \\
\arrayrulecolor{gray!30}\cmidrule(lr){2-11}\arrayrulecolor{black}
 & cov@1   & 0.0396                   & 0.0337                   & \underline{0.0409}       & 0.0363                   & 0.0356                   & 0.0369                   & 0.0387                   & \textbf{0.0440* $ \pm $ 0.0005} & +7.6\% \\
 & cov@5   & 0.1278                   & 0.1076                   & \underline{0.1492}       & 0.1077                   & 0.1123                   & 0.1082                   & 0.1304                   & \textbf{0.1665* $ \pm $ 0.0019} & +11.6\% \\
 & cov@10  & 0.1920                   & 0.1665                   & \underline{0.2346}       & 0.1598                   & 0.1719                   & 0.1703                   & 0.2016                   & \textbf{0.2673* $ \pm $ 0.0021} & +13.9\% \\
    \bottomrule
\end{tabular}
    }

    \label{table:utility_metrics}
\end{table*}


==> recsys26-115/Source/tables/yelp_abol.tex <==
\begin{figure}[!t]
    \centering

    % ─── first row ─────────────────────────────────────────────
    \includegraphics[width=1\linewidth]{pictures/ablation/alpha_diversity_tradeoff.png}
    %\includegraphics[width=0.49\linewidth]{pictures/ablation/yelp_lambda_1_buckets_hr.png}
    
    \caption{Parameter sensitivity wrt $\alpha$ for YELP dataset. Left: common metrics, Right: item-popularity bucket metrics. Picture demonstrates controllability of recommendations via hyperparameter. }
    \label{figure:yelp_abol}
\end{figure}

==> recsys26-115/Source/tables/yelp_alignment.tex <==
\begin{figure}[!t]
    \centering

    % ─── first row ─────────────────────────────────────────────
    \includegraphics[width=1\linewidth]{pictures/alignment/yelp.png}
    %\includegraphics[width=0.49\linewidth]{pictures/ablation/yelp_lambda_1_buckets_hr.png}
    
    \caption{Alignment Concentration on YELP dataset. (left) We plot each model in relative alignment, $\tilde g_b$, coordinates. (right) AC score accumulates how much more head bucket items are aligned to global user embedding compared to less popular buckets.}
    \label{figure:yelp_alignment}
\end{figure}

==> tables/ablation_buckets_fig.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_1_buckets_hr.png}
    \caption{Sensitivity Analysis w.r.t. $ \alpha $ for recommendations over 3 item popularity buckets}
    \label{figure:ablation_alpha_buckets}
\end{figure*}

==> tables/ablation_lambda_buckets_fig.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_2_buckets_hr.png}
    \caption{Sensitivity Analysis w.r.t. $ \lambda $ for recommendations over 3 item popularity buckets}
    \label{figure:ablation_lambda_buckets}
\end{figure*}

==> tables/ablation_lambda_main_fig.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_2_HR.png}
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_2_cov.png}
    \caption{Sensitivity Analysis w.r.t. $ \lambda $ of hr@K and cov@K metrics }
    \label{figure:ablation_lambda_main}
\end{figure*}

==> tables/ablation_main_fig.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_1_HR.png}
    \includegraphics[width=0.99\linewidth]{pictures/ablation/lambda_1_cov.png}
    \caption{Sensitivity Analysis w.r.t. $ \alpha $ of hr@K and cov@K metrics }
    \label{figure:ablation_main}
\end{figure*}

==> tables/compare_buckets_table.tex <==
\begin{table}[!t]
    \centering
    \caption{Integral metric for Figure 4}
    \begin{tabular}{c|c c c}
        \toprule
          & SASRec(BCE) & BT-SR( $ \alpha = 0.1 $ ) & BT-SR( $ \alpha = 0.4 $ ) \\ 
         \toprule
         \textbf{ndcg@20} & 0.0176 & 0.0180 & 0.0182 \\
         \toprule
    \end{tabular}
    \label{tab:pop_buckets_ndcg}
\end{table}

==> tables/mixed_fig.tex <==
\begin{figure}[!t]
    \centering

    \includegraphics[width=0.5\linewidth]{pictures/scores_density/MovieLens_1M.png}
    \includegraphics[width=0.49\linewidth]{pictures/spectrum/MovieLens_1M.png}
    
    \includegraphics[width=0.49\linewidth]{pictures/scores_density/YELP.png}
    \includegraphics[width=0.49\linewidth]{pictures/spectrum/YELP.png}
    
    \includegraphics[width=0.5\linewidth]{pictures/scores_density/Gowalla.png}
    \includegraphics[width=0.49\linewidth]{pictures/spectrum/Gowalla.png}
    
    \caption{(left) Comparison of score density distributions for positive and negative candidate pairs across three datasets. We quantify model’s confidence in distinguishing relevant candidates by the histogram overlap factor (\emph{Overlap})—lower values indicate better separation. (right) Singular value spectra of the sequence embeddings for each dataset, annotated with their computed effective ranks (in legend), illustrate the effective dimensionality of the learned representations. }
    \label{figure:scores_dens_fig}
    %\\[-10pt]
\end{figure}

==> tables/old_met.tex <==
\begin{table*}[!ht]
    \caption{Performance comparison across all datasets.Bold scores are the best on the dataset for the given metric,underlined scores are the second best.}
    {\tiny
    \begin{tabular}{rlcccccccl}
    \toprule
    Dataset & Metric & SasRec(BCE) & SasRec(CE) & SasRec(SCE) & CL4SRec & DuoRec & EC4SRec & BT-SR & Improve \\
    \midrule
    \multirow{9}{*}{ML 1M}
     & hr@1 & 0.0160 & \underline{0.0213} & 0.0200 & 0.0182 & 0.0200 & 0.0213 & \textbf{0.0293} & +37.6\% \\
     & hr@5   & 0.0493 & 0.0600 & \underline{0.0587} & 0.0476 & 0.0480 & 0.0534 & \textbf{0.0600} & +0.0\%  \\
     & hr@10  & 0.0893 & 0.0880 & \underline{0.0933} & 0.0834 & 0.0800 & 0.0880 & \textbf{0.0987} & +5.8\%  \\
     & ndcg@5 & 0.0319 & \underline{0.0404} & 0.0393 & 0.0342 & 0.0353 & 0.0364 & \textbf{0.0461} & +14.1\% \\
     & ndcg@10& 0.0443 & 0.0494 & \underline{0.0503} & 0.0464 & 0.0456 & 0.0492 & \textbf{0.0583} & +15.9\% \\
     & ndcg@50& 0.0799 & \underline{0.0818} & 0.0800 & 0.0712 & 0.0723 & 0.0748 & \textbf{0.0871} & +6.5\%  \\
     & cov@1  & 0.0320 & \underline{0.0887} & \textbf{0.0961} & 0.0335 & 0.0361 & 0.0387 & 0.0849 & -11.7\% \\
     & cov@5  & 0.1473 & 0.2265 & \textbf{0.2568} & 0.0969 & 0.0936 & 0.1002 & \underline{0.2327} & -9.4\% \\
     & cov@10 & 0.2434 & 0.3185 & \textbf{0.3645} & 0.1329 & 0.1459 & 0.1591 & \underline{0.3242} & -11.1\% \\
    \midrule
    \multirow{9}{*}{YELP}
     & hr@1   & \underline{0.0045} & 0.0043 & 0.0040 & 0.0028 & 0.0027 & 0.0028 & \textbf{0.0049} & +8.9\% \\
     & hr@5   & \underline{0.0162} & 0.0137 & 0.0152 & 0.0087 & 0.0094 & 0.0090 & \textbf{0.0183} & +13.0\% \\
     & hr@10  & 0.0292 & 0.0257 & 0.0277 & 0.0192 & 0.0188 & \underline{0.0199} & \textbf{0.0288} & -1.4\% \\
     & ndcg@5 & \underline{0.0104} & 0.0088 & 0.0097 & 0.0060 & 0.0061 & 0.0062 & \textbf{0.0117} & +12.5\% \\
     & ndcg@10& \underline{0.0146} & 0.0127 & 0.0137 & 0.0085 & 0.0091 & 0.0092 & \textbf{0.0150} & +2.7\%  \\
     & ndcg@50& \textbf{0.0280} & 0.0263 & 0.0258 & 0.0178 & 0.0172 & \underline{0.0184} & 0.0267 & -4.6\%  \\
     & cov@1  & 0.0103 & \textbf{0.0233} & 0.0135 & 0.0057 & 0.0059 & 0.0059 & \underline{0.0218} & -6.4\%  \\
     & cov@5  & 0.0333 & \underline{0.0621} & 0.0413 & 0.0170 & 0.0161 & 0.0171 & \textbf{0.0636} & +2.4\%  \\
     & cov@10 & 0.0541 & \underline{0.0911} & 0.0661 & 0.0276 & 0.0255 & 0.0275 & \textbf{0.0998} & +9.5\% \\
    \midrule
    \multirow{9}{*}{Gowalla}
     & hr@1   & 0.0173 & 0.0143 & \underline{0.0196} & 0.0157 & 0.0144 & 0.0142 & \textbf{0.0205} & +4.6\%  \\
     & hr@5   & 0.0506 & 0.0431 & \underline{0.0548} & 0.0433 & 0.0473 & 0.0440 & \textbf{0.0592} & +8.0\%  \\
     & hr@10  & 0.0756 & 0.0660 & \underline{0.0811} & 0.0694 & 0.0712 & 0.0757 & \textbf{0.0851} & +4.9\%  \\
     & ndcg@5 & 0.0339 & 0.0289 & \underline{0.0372} & 0.0318 & 0.0310 & 0.0331 & \textbf{0.0400} & +7.5\%  \\
     & ndcg@10& 0.0419 & 0.0364 & \underline{0.0457} & 0.0411 & 0.0387 & 0.0397 & \textbf{0.0483} & +5.7\%  \\
     & ndcg@50& 0.0613 & 0.0528 & \underline{0.0640} & 0.0535 & 0.0587 & 0.0549 & \textbf{0.0667} & +4.2\%  \\
     & cov@1  & 0.0230 & 0.0228 & 0.0214 & 0.0252 & \underline{0.0255} & 0.0270 & \textbf{0.0321} & +25.9\% \\
     & cov@5  & 0.0892 & 0.0725 & 0.0921 & \underline{0.0950} & 0.0939 & 0.0998 & \textbf{0.1280} & +36.3\% \\
     & cov@10 & 0.1557 & 0.1153 & \underline{0.1625} & 0.1538 & 0.1595 & 0.1650 & \textbf{0.2187} & +34.6\% \\
    \midrule
    \multirow{9}{*}{Beauty}
     & hr@1   & 0.0179 & 0.0269 & \underline{0.0305} & 0.0292 & 0.0305 & 0.0312 & \textbf{0.0314} & +3.0\%  \\
     & hr@5   & 0.0538 & \underline{0.0591} & 0.0582 & 0.0555 & 0.0573 & 0.0574 & \textbf{0.0618} & +4.6\%  \\
     & hr@10  & 0.0789 & 0.0896 & \underline{0.0905} & 0.0830 & 0.0860 & 0.0815 & \textbf{0.0941} & +4.0\%  \\
     & ndcg@5 & 0.0355 & 0.0425 & \underline{0.0442} & 0.0412 & 0.0436 & 0.0455 & \textbf{0.0460} & +4.1\%  \\
     & ndcg@10& 0.0434 & 0.0524 & \underline{0.0543} & 0.0530 & 0.0527 & 0.0557 & \textbf{0.0563} & +3.7\%  \\
     & ndcg@50& 0.0659 & 0.0777 & \underline{0.0794} & 0.0833 & 0.0789 & 0.0794 & \textbf{0.0829} & +4.4\%  \\
     & cov@1  & 0.0620 & 0.0546 & 0.0499 & 0.0603 & \underline{0.0607} & \textbf{0.0679} & 0.0492 & -20.6\% \\
     & cov@5  & 0.2200 & 0.1782 & 0.1760 & \underline{0.2212} & 0.2100 & 0.2103 & \textbf{0.1562} & -29.0\% \\
     & cov@10 & 0.3448 & 0.2752 & 0.2766 & \underline{0.3362} & 0.3234 & 0.3236 & \textbf{0.2397} & -30.5\% \\
    \midrule
    \multirow{9}{*}{Kindle Store}
     & hr@1   & 0.0451 & 0.0471 & \underline{0.0533} & 0.0469 & 0.0471 & 0.0505 & \textbf{0.0565} & +6.0\%  \\
     & hr@5   & 0.0832 & 0.0813 & \underline{0.0899} & 0.0813 & 0.0762 & 0.0785 & \textbf{0.0916} & +1.9\%  \\
     & hr@10  & 0.0990 & 0.0965 & \underline{0.1022} & 0.0910 & 0.0897 & 0.0955 & \textbf{0.1043} & +2.1\%  \\
     & ndcg@5 & 0.0655 & 0.0652 & \underline{0.0726} & 0.0635 & 0.0625 & 0.0652 & \textbf{0.0755} & +4.0\%  \\
     & ndcg@10& 0.0705 & 0.0700 & \underline{0.0765} & 0.0662 & 0.0668 & 0.0672 & \textbf{0.0796} & +4.1\%  \\
     & ndcg@50& 0.0786 & 0.0803 & \underline{0.0852} & 0.0731 & 0.0771 & 0.0736 & \textbf{0.0886} & +4.0\%  \\
     & cov@1  & 0.0396 & 0.0337 & \underline{0.0409} & 0.0363 & 0.0356 & 0.0369 & \textbf{0.0433} & +5.9\%  \\
     & cov@5  & 0.1278 & 0.1076 & \underline{0.1492} & 0.1077 & 0.1123 & 0.1082 & \textbf{0.1656} & +11.0\% \\
     & cov@10 & 0.1920 & 0.1665 & \underline{0.2346} & 0.1598 & 0.1719 & 0.1703 & \textbf{0.2665} & +13.6\% \\
    \bottomrule
    \end{tabular}
    }
    \label{table:utility_metrics}
\end{table*}










\begin{figure*}[!t]
    \centering

    % ─── first row ─────────────────────────────────────────────
    \includegraphics[width=0.33\linewidth]{pictures/bucket_metrics/ml.png}
    \includegraphics[width=0.33\linewidth]{pictures/bucket_metrics/yelp.png}
    \includegraphics[width=0.32\linewidth]{pictures/bucket_metrics/gowalla.png}%
    \\[-40pt] % ← tighten vertical space (adjust value to taste)

    % ─── second row ────────────────────────────────────────────
    \includegraphics[width=0.33\linewidth]{pictures/bucket_metrics/ml_hr10.png}
    \includegraphics[width=0.33\linewidth]{pictures/bucket_metrics/yelp_hr10.png}
    \includegraphics[width=0.32\linewidth]{pictures/bucket_metrics/gowalla_hr10.png}
    \\[-40pt]
    
    \caption{Item-popularity-bucket HR@1 and HR@10 metrics across three datasets}
    \label{figure:pop_buckets}
\end{figure*}

==> tables/projections.tex <==
\begin{figure}[!t]
    %\\[-5pt]
    \centering
    \includegraphics[width=0.99\linewidth]{pictures/projections/seq_yelp.png}
    \includegraphics[width=0.99\linewidth]{pictures/projections/seq_ml1m.png}
    \caption{UMAP of sequence embeddings from BT-ST (ours), SasRec (CE; base model), and DuoRec (contrastive SR) on Yelp (top row) and MovieLens 1M (bottom row). On Yelp, BT-ST produces more dispersed, sparser clusters. On MovieLens 1M, it yields fewer, tighter clusters with higher density.}
    \label{figure:seq_2d_yelp}
    %\\[-15pt]
\end{figure}

==> tables/scores_dens_fig.tex <==
\begin{figure}[!ht]
    \centering

    \includegraphics[width=0.5\linewidth]{pictures/scores_density/MovieLens 1M.png}
    \includegraphics[width=0.5\linewidth]{pictures/spectrum/MovieLens 1M.png}
    
    \includegraphics[width=0.49\linewidth]{pictures/scores_density/YELP.png}
    \includegraphics[width=0.49\linewidth]{pictures/spectrum/YELP.png}
    
    \includegraphics[width=0.5\linewidth]{pictures/scores_density/Gowalla.png}
    \includegraphics[width=0.5\linewidth]{pictures/spectrum/Gowalla.png}
    
    \caption{Scores densities comparison for positives and negatives candidates on 3 datasets. To estimate confidence of relevant candidates we computed histograms overlap factor between positives and negatives(Overlap). Lower overlap is better }
    \label{figure:scores_dens_fig}
\end{figure}

==> tables/spectrum_fig.tex <==
\begin{figure}[!ht]
    \\[-10pt]
    \centering
    \includegraphics[width=0.5\linewidth]{pictures/spectrum/MovieLens 1M.png}
    \includegraphics[width=0.49\linewidth]{pictures/spectrum/YELP.png}
    \includegraphics[width=0.5\linewidth]{pictures/spectrum/Gowalla.png}
    
    \caption{Sequence embeddings singular values across multiple datasets with stable rank}
    \label{figure:spectrums}
\end{figure}

==> tables/yelp_abol.tex <==
\begin{figure}[!t]
    \centering

    % ─── first row ─────────────────────────────────────────────
    \includegraphics[width=1\linewidth]{pictures/ablation/alpha_diversity_tradeoff.png}
    %\includegraphics[width=0.49\linewidth]{pictures/ablation/yelp_lambda_1_buckets_hr.png}
    
    \caption{Parameter sensitivity wrt $\alpha$ for YELP dataset. Left: common metrics, Right: item-popularity bucket metrics. Picture demonstrates controllability of recommendations via hyperparameter. }
    \label{figure:yelp_abol}
\end{figure}

==> tables/yelp_alignment.tex <==
\begin{figure}[!t]
    \centering

    % ─── first row ─────────────────────────────────────────────
    \includegraphics[width=1\linewidth]{pictures/alignment/yelp.png}
    %\includegraphics[width=0.49\linewidth]{pictures/ablation/yelp_lambda_1_buckets_hr.png}
    
    \caption{Alignment Concentration on YELP dataset. (left) We plot each model in relative alignment, $\tilde g_b$, coordinates. (right) AC score accumulates how much more head bucket items are aligned to global user embedding compared to less popular buckets.}
    \label{figure:yelp_alignment}
\end{figure}
